Probably Approximately Correct Nonlinear Model Predictive Control (PAC-NMPC)

Approaches for stochastic nonlinear model predictive control (SNMPC) typically make restrictive assumptions about the system dynamics and rely on approximations to characterize the evolution of the underlying uncertainty distributions. For this reason, they are often unable to capture more complex distributions (e.g., non-Gaussian or multi-modal) and cannot provide accurate guarantees of performance. In this paper, we present a sampling-based SNMPC approach that leverages recently derived sample complexity bounds to certify the performance of a feedback policy without making assumptions about the system dynamics or underlying uncertainty distributions. By parallelizing our approach, we are able to demonstrate real-time receding-horizon SNMPC with statistical safety guarantees in simulation and on hardware using a 1/10th scale rally car and a 24-inch wingspan fixed-wing unmanned aerial vehicle (UAV).

==> old_fixedwing.tex <==
\section{Application to Fixed-Wing UAVs}

TODO: Add fixed-wing hardware experiment to this section. 

\subsection{Setup}

To demonstrate that our approach can extend to more complex, high-dimensional systems, we use PAC-NMPC to control a simulated fixed-wing dynamical system. We simulate a quaternion formulation of the fixed-wing described in \cite{basescu2020direct} with RK2 integration. This system has a 17-dimensional state space and a 4-dimensional control space. We place zero-mean Gaussian noise over the dynamics with a covariance of 

{\footnotesize
\begin{align}
  \vectg{\Sigma} = diag([.001, .001, .001, .001, .001, .001, .001, \nonumber \\ .1, .1, .1, 5, 5, 5, 25, 25, 25, .001]) \nonumber
\end{align}
}%

We optimize a 12 timestep trajectory with $\Delta t = 0.1$ sec at a replanning period of $H = 0.2$. We apply a quadratic cost of the form $J = \vect{x_T}^T\vect{Q_f}\vect{x_T} + \sum_{i=1}^{T-1} \vect{x_i}^T\vect{Q}\vect{x_i}$ and an obstacle constraint. Parameters were as follows: $L=1$, $M=1024$, $\delta=0.05$, and $\gamma=10$. We use feedback and use stochastic dynamics to optimize the PAC bounds. The state costs were:

{\footnotesize
\begin{align}
    \vect{Q} = diag([0, 0, 0, 0, 0, 0, 0, .1, .1, .1, 0, 0, 0, 0, 0, 0, 0])\nonumber \\
    \vect{Q_f} = diag([.1, .1, .1, .5, .5, .5, .5, .1, .1, .1, .01, .01, .01, .01, .01, .01, 0])\nonumber
\end{align}
}%

The TVLQR costs were:

{\footnotesize
\begin{align}
    \vect{Q'} = diag([25, 25, 25, 50, 50, 50, 50, 2, 2, 2, 2, 2, 2, 2, 2, 2, 2])\nonumber \\
    \vect{Q_f'} = diag([100, 100, 100, 100, 100, 100, 100, 1, 1, 1, 1, 1, 1, 1, 1, 1, 1])\nonumber\\
    \vect{R'} = diag(1, 1, 1, 25)\nonumber
\end{align}
}%

To enable real time performance, we compute the linearized dynamics for the feedback policy using finite difference on the mean trajectory of the latest prior distribution. This still results in valid PAC bounds since the number of prior policies, $L$, is set to one. This simulation was run on a desktop computer with an AMD Ryzen 7 5800x and a NVIDIA GeForce RTX 3080.

\subsection{Results}

PAC-NMPC was successfully able to control the simulated fixed-wing in real time, following the path while avoiding nearby obstacles. In Figure \ref{fig:uav_nmpc_route}, we display the route taken by the system during five loops of the path.

\begin{figure}[t]%
    \centering
      \includegraphics[trim={15 20 45 55},clip,width=.75\columnwidth]{images/uav_nmpc_route.pdf}
      \caption{Path taken while following route (black) and avoiding obstacles (brown) with fixed-wing simulation.}
    \label{fig:uav_nmpc_route}
\end{figure}

During each planning interval of $H = 0.2$ sec, the controller achieved an average of 24 iterations of trajectory distribution optimization (approximately 8.3ms per iteration). The controller consistently produced PAC bounds of less than 15\% probability of collision, which accurately bounded the Monte Carlo estimates (Fig. \ref{fig:uav_nmpc_bound}).

\begin{figure}[t]%
    \centering
      \includegraphics[trim={5 0 45 20}, clip, width=.75\columnwidth]{images/uav_nmpc_bound.pdf}
      \caption{Optimized PAC Bound compared to Monte Carlo estimates for probability of constraint violation.}
    \label{fig:uav_nmpc_bound}
\end{figure}
